Solar Multimodal Transformer: Intraday Solar Irradiance Predictor using Public Cameras and Time Series

Accurate intraday solar irradiance forecasting is crucial for optimizing dispatch planning and electricity trading. For this purpose, we introduce a novel and effective approach that includes three distinguishing components from the literature: 1) the uncommon use of single-frame public camera imagery; 2) solar irradiance time series scaled with a proposed normalization step, which boosts performance; and 3) a lightweight multimodal model, called Solar Multimodal Transformer (SMT), that delivers accurate short-term solar irradiance forecasting by combining images and scaled time series. Benchmarking against Solcast, a leading solar forecasting service provider, our model improved prediction accuracy by 25.95%. Our approach allows for easy adaptation to various camera specifications, offering broad applicability for real-world solar forecasting challenges.

==> Tables/table_results_main.tex <==

\begin{table}[ht]
\centering
\label{tab:model_comparison}
\begin{tabular}{>{\raggedright}p{3cm} >{\raggedright\arraybackslash}p{2.2cm} >{\raggedright\arraybackslash}p{7cm}}
\toprule
\textbf{Input Data} & \textbf{Preprocessing} & \textbf{Model Structure} &\textbf{RMSE} &\textbf{RSE} \\
\midrule
img & - & CNN \\
img & - & CNN+LSTM \\
img & - & Transformer \\
ts & - & CNN+GRU  \\
ts & - & Transformer \\
img + ts & - & CNN+LSTM (img) + CNN+GRU(ts) \\
img + ts & - & Unet (img) + CNN+GRU(ts) \\
img + ts & - & Transformer \\
img(2 camera) + ts & - & Transformer \\
img + ts + smart token & - & Transformer \\
img + ts & CNN (img) & Transformer \\
img + ts & Unet (img) & Transformer \\
\bottomrule
\end{tabular}
\caption{Comparison of Model Architectures: All the models are tested on the same period, from 28 September 2023 until 29 Janurary 2024, as well as 27 March 2023 to 11 April 2023 for the comparison with Solcast. We report mean and standard deviation of rmse and scaled rmse across 10 bootstrapping runnings by resampling the training data with replacement, i.e. around 63.2\% of training data is used during each run.}
\end{table}
